Implications of time-dependent molecular chemistry in metal-poor dwarf stars

Binary molecules such as CO, OH, CH, CN, and C$_2$ are often used as abundance indicators in stars. These species are usually assumed to be formed in chemical equilibrium. The time-dependent effects of hydrodynamics can affect the formation and dissociation of these species and may lead to deviations from chemical equilibrium. We aim to model departures from chemical equilibrium in dwarf stellar atmospheres by considering time-dependent chemical kinetics alongside hydrodynamics and radiation transfer. We examine the effects of a decreasing metallicity and an altered C/O ratio on the chemistry when compared to the equilibrium state. We used the radiation-(magneto)hydrodynamics code CO5BOLD, and its own chemical solver to solve for the chemistry of 15 species and 83 reactions. The species were treated as passive tracers and were advected by the velocity field. The steady-state chemistry was also computed to isolate the effects of hydrodynamics. In most of the photospheres in the models we present, the mean deviations are smaller than $0.2$ dex, and they generally appear above $\log{\tau} = -2$. The deviations increase with height because the chemical timescales become longer with decreasing density and temperature. A reduced metallicity similarly results in longer chemical timescales and in a reduction in yield that is proportional to the drop in metallicity; a decrease by a factor $100$ in metallicity loosely corresponds to an increase by factor $100$ in chemical timescales. As both CH and OH are formed along reaction pathways to CO, the C/O ratio means that the more abundant element gives faster timescales to the constituent molecular species. Overall, the carbon enhancement phenomenon seen in very metal-poor stars is not a result of an improper treatment of molecular chemistry for stars up to a metallicity as low as [Fe/H] = $-3.0$.

==> tables/cemp_models.tex <==
% Table with model ID, Teff, logg, metallicity, resolution, extent,
% carbon & oxygen abundance & C/O
\begin{table}[h!]
  \begin{center}
    \scalebox{0.87}{
      \begin{tabular}{ l r c c r r r l}
        \toprule
        Model ID & [Fe/H]  & A(C)   & A(O)   & $\log$ C / O & Internal ID   \\
        \midrule
                 &         &        &        &              & (d3t63g40)    \\
        \midrule
        AM1      & $+0.00$ & $8.41$ & $8.66$ & $-0.25$      & mm00          \\
        AM2      & $-2.00$ & $6.41$ & $7.06$ & $-0.65$      & mm20          \\
        AM3      & $-3.00$ & $5.41$ & $6.06$ & $-0.65$      & mm30          \\
        \midrule
        AC1      & $-3.00$ & $7.39$ & $7.66$ & $-0.27$      & mm30c20n20o20 \\
        AC2      & $-3.00$ & $7.39$ & $6.06$ & $+1.33$      & mm30c20n20o04 \\
        \midrule
        % d3t40g15mm00          & 4000      & 1.50                & +0.00  & 8.43                     & 8.69 &       \\
        % d3t40g15mm20          & 4000      & 1.50                & -2.00  & 6.41                     & 7.06 &       \\
        % d3t40g16mm30          & 4000      & 1.50                & -3.00  & 5.41                     & 6.06 &       \\
        % \midrule
        % d3t50g16mm00          & 5000      & 1.60                & +0.00  & 8.43                     & 8.69 &       \\
        % d3t50g16mm20          & 5000      & 1.60                & -2.00  & 6.41                     & 7.06 &       \\
        % d3t50g16mm30          & 5000      & 1.60                & -3.00  & 5.41                     & 6.06 &       \\
        % \midrule
        % d3t36g10mm00          & 3600      & 1.00                & +0.00  & 8.43                     & 8.69 &       \\
        \bottomrule
      \end{tabular}
    }
  \end{center}
  \caption{Model atmosphere parameters for the five models used in the study.
    Each model has $\Teff = 6250$ K and $\log{g} = 4.00$, a resolution of
    $140\times140\times150$ cells and an extent of $26\times26\times12.7$ Mm
    ($x\,\times\,y\,\times\,z$). The abundances
    for each model are consistent with those in the respective opacity tables,
    and we use the ``Internal ID'' to refer to each model uniquely within this
    work.}
  \label{table:model_overview}
\end{table}

==> tables/cno_table.tex <==
\onecolumn
\begin{longtable}{r l c l r r r r}
      \caption{
            Reactions used in this work. ``Index'' refers to the index in the UMIST
            astrochemistry database. All reactions are of modified-Arrhenius form with
            rate coefficient
            $k(T) = \alpha \left(\frac{T}{300}\right)^\beta \exp\left(\frac{-\gamma}{T}\right)$.
            References are:
            % ``UMIST99'' \citet{leteuffUMISTDatabase2000},
            ``UMIST'' \citet{mcelroyUMISTDatabase2013}
            ``BDHL72'' \citet{baulchEvaluatedKinetic1972},
            ``KCD'' \citet{konnov2000},
            ``BDDG76'' \citet{baulchEvaluatedKinetic1976},
            ``W80'' \citet{westleyTableRecommended1980}
      }                                                                                                                                          \\                                                                                                            \\                                                                                                                            \\
      \hline
      Index & Reactants                      &                          & Products                   & $\alpha$ & $\beta$ & $\gamma$ & Reference \\
      \hline
            &                                & Radiative Association    &                            &          &         &          &           \\
      \hline
      3681  & C   +             H            & $\Longrightarrow$        & CH       + $\gamma$        & 1.00e-17 & 0.00    & 0.0      & UMIST     \\
      3683  & H   +             O            & $\Longrightarrow$        & OH       + $\gamma$        & 9.90e-19 & -0.38   & 0.0      & UMIST     \\
      3703  & C   +             C            & $\Longrightarrow$        & C$_2$    + $\gamma$        & 4.36e-18 & 0.35    & 161.3    & UMIST     \\
      3705  & C   +             N            & $\Longrightarrow$        & CN       + $\gamma$        & 5.72e-19 & 0.37    & 51.0     & UMIST     \\
      3707  & C   +             O            & $\Longrightarrow$        & CO       + $\gamma$        & 1.58e-17 & 0.34    & 1297.0   & UMIST     \\
      3730  & O   +             O            & $\Longrightarrow$        & O$_2$    + $\gamma$        & 4.90e-20 & 1.58    & 0.0      & UMIST     \\
      \hline
            &                                & 3-body association       &                            &          &         &          &           \\
      \hline
      4079  & H   +             M   +  O     & $\Longrightarrow$        & M   +         OH           & 4.33e-32 & -1.00   & 0.0      & UMIST     \\
      4097  & C   +             M   +  O     & $\Longrightarrow$        & CO  +         M            & 2.14e-29 & -3.08   & -2114.0  & BDDG76    \\
      5000  & H   +             H   +  M     & $\Longrightarrow$        & H$_2$  +         M         & 6.43e-33 & -1.00   & 0.0      & KCD       \\
      5001  & H   +             H   +  H$_2$ & $\Longrightarrow$        & H$_2$  +         H$_2$     & 9.00e-33 & -0.60   & 0.0      & KCD       \\
      5002  & H   +             H   +  H     & $\Longrightarrow$        & H   +         H$_2$        & 4.43e-28 & -4.00   & 0.0      & BDHL72    \\
      7000  & H   +             H   +  O     & $\Longrightarrow$        & H   +         OH           & 1.00e-32 & 0.00    & 0.0      & BDHL72    \\
      7001  & C   +             H   +  O     & $\Longrightarrow$        & CO  +         H            & 2.14e-29 & -3.08   & -2114.0  & BDDG76    \\
      \hline
            &                                & Species Exchange         &                            &          &         &          &           \\
      \hline
      1     & CH  +             H            & $\Longrightarrow$        & C   +         H$_2$        & 2.70e-11 & 0.38    & 0.0      & UMIST     \\
      3     & H   +             NH           & $\Longrightarrow$        & H$_2$  +         N         & 1.73e-11 & 0.50    & 2400.0   & UMIST     \\
      8     & H   +             OH           & $\Longrightarrow$        & H$_2$  +         O         & 6.99e-14 & 2.80    & 1950.0   & UMIST     \\
      11    & C$_2$  +             H         & $\Longrightarrow$        & C   +         CH           & 4.67e-10 & 0.50    & 30450.0  & UMIST     \\
      14    & CO  +             H            & $\Longrightarrow$        & C   +         OH           & 5.75e-10 & 0.50    & 77755.0  & W80       \\
      18    & H   +             NO           & $\Longrightarrow$        & NH  +         O            & 9.29e-10 & -0.10   & 35220.0  & UMIST     \\
      19    & H   +             NO           & $\Longrightarrow$        & N   +         OH           & 3.60e-10 & 0.00    & 24910.0  & UMIST     \\
      24    & H   +             O$_2$        & $\Longrightarrow$        & O   +         OH           & 2.61e-10 & 0.00    & 8156.0   & UMIST     \\
      42    & C   +             H$_2$        & $\Longrightarrow$        & CH  +         H            & 6.64e-10 & 0.00    & 11700.0  & UMIST     \\
      44    & H$_2$  +             N         & $\Longrightarrow$        & H   +         NH           & 1.69e-09 & 0.00    & 18095.0  & UMIST     \\
      48    & H$_2$  +             O         & $\Longrightarrow$        & H   +         OH           & 3.14e-13 & 2.70    & 3150.0   & UMIST     \\
      52    & H$_2$  +             O$_2$     & $\Longrightarrow$        & OH  +         OH           & 3.16e-10 & 0.00    & 21890.0  & UMIST     \\
      58    & C   +             CH           & $\Longrightarrow$        & C$_2$  +         H         & 6.59e-11 & 0.00    & 0.0      & UMIST     \\
      61    & C   +             NH           & $\Longrightarrow$        & CH  +         N            & 1.73e-11 & 0.50    & 4000.0   & UMIST     \\
      62    & C   +             NH           & $\Longrightarrow$        & CN  +         H            & 1.20e-10 & 0.00    & 0.0      & UMIST     \\
      66    & C   +             OH           & $\Longrightarrow$        & CH  +         O            & 2.25e-11 & 0.50    & 14800.0  & UMIST     \\
      67    & C   +             OH           & $\Longrightarrow$        & CO  +         H            & 1.81e-11 & 0.50    & 0.0      & W80       \\
      68    & C   +             CN           & $\Longrightarrow$        & C$_2$  +         N         & 4.98e-10 & 0.00    & 18116.0  & UMIST     \\
      70    & C   +             CO           & $\Longrightarrow$        & C$_2$  +         O         & 2.94e-11 & 0.50    & 58025.0  & UMIST     \\
      71    & C   +             N$_2$        & $\Longrightarrow$        & CN  +         N            & 8.69e-11 & 0.00    & 22600.0  & UMIST     \\
      75    & C   +             NO           & $\Longrightarrow$        & CN  +         O            & 6.00e-11 & -0.16   & 0.0      & UMIST     \\
      76    & C   +             NO           & $\Longrightarrow$        & CO  +         N            & 9.00e-11 & -0.16   & 0.0      & UMIST     \\
      80    & C   +             O$_2$        & $\Longrightarrow$        & CO  +         O            & 5.56e-11 & 0.41    & -26.9    & UMIST     \\
      100   & CH  +             N            & $\Longrightarrow$        & C   +         NH           & 3.03e-11 & 0.65    & 1207.0   & UMIST     \\
      102   & CH  +             O            & $\Longrightarrow$        & C   +         OH           & 2.52e-11 & 0.00    & 2381.0   & UMIST     \\
      104   & CH  +             O            & $\Longrightarrow$        & CO  +         H            & 1.02e-10 & 0.00    & 914.0    & UMIST     \\
      116   & CH  +             O$_2$        & $\Longrightarrow$        & CO  +         OH           & 7.60e-12 & 0.00    & 0.0      & UMIST     \\
      126   & N   +             NH           & $\Longrightarrow$        & H   +         N$_2$        & 4.98e-11 & 0.00    & 0.0      & UMIST     \\
      130   & N   +             OH           & $\Longrightarrow$        & NH  +         O            & 1.88e-11 & 0.10    & 10700.0  & UMIST     \\
      131   & N   +             OH           & $\Longrightarrow$        & H   +         NO           & 6.05e-11 & -0.23   & 14.9     & UMIST     \\
      132   & C$_2$  +             N         & $\Longrightarrow$        & C   +         CN           & 5.00e-11 & 0.00    & 0.0      & UMIST     \\
      133   & CN  +             N            & $\Longrightarrow$        & C   +         N$_2$        & 1.00e-10 & 0.40    & 0.0      & UMIST     \\
      138   & N   +             NO           & $\Longrightarrow$        & N$_2$  +         O         & 3.38e-11 & -0.17   & -2.8     & UMIST     \\
      144   & N   +             O$_2$        & $\Longrightarrow$        & NO  +         O            & 2.26e-12 & 0.86    & 3134.0   & UMIST     \\
      195   & NH  +             NH           & $\Longrightarrow$        & H$_2$  +         N$_2$     & 1.70e-11 & 0.00    & 0.0      & UMIST     \\
      197   & NH  +             O            & $\Longrightarrow$        & N   +         OH           & 1.16e-11 & 0.00    & 0.0      & UMIST     \\
      198   & NH  +             O            & $\Longrightarrow$        & H   +         NO           & 1.80e-10 & 0.00    & 300.0    & UMIST     \\
      206   & NH  +             NO           & $\Longrightarrow$        & N$_2$  +         OH        & 1.46e-11 & -0.58   & 37.0     & UMIST     \\
      236   & O   +             OH           & $\Longrightarrow$        & H   +         O$_2$        & 1.77e-11 & 0.00    & -178.0   & UMIST     \\
      240   & C$_2$  +             O         & $\Longrightarrow$        & C   +         CO           & 2.00e-10 & -0.12   & 0.0      & UMIST     \\
      243   & CN  +             O            & $\Longrightarrow$        & C   +         NO           & 5.37e-11 & 0.00    & 13800.0  & UMIST     \\
      244   & CN  +             O            & $\Longrightarrow$        & CO  +         N            & 5.00e-11 & 0.00    & 200.0    & UMIST     \\
      251   & N$_2$  +             O         & $\Longrightarrow$        & N   +         NO           & 2.51e-10 & 0.00    & 38602.0  & UMIST     \\
      261   & NO  +             O            & $\Longrightarrow$        & N   +         O$_2$        & 1.18e-11 & 0.00    & 20413.0  & UMIST     \\
      377   & C$_2$  +             O$_2$     & $\Longrightarrow$        & CO  +         CO           & 1.50e-11 & 0.00    & 4300.0   & UMIST     \\
      382   & CN  +             CN           & $\Longrightarrow$        & C$_2$  +         N$_2$     & 2.66e-09 & 0.00    & 21638.0  & UMIST     \\
      387   & CN  +             NO           & $\Longrightarrow$        & CO  +         N$_2$        & 1.60e-13 & 0.00    & 0.0      & UMIST     \\
      392   & CN  +             O$_2$        & $\Longrightarrow$        & CO  +         NO           & 5.12e-12 & -0.49   & -5.2     & UMIST     \\
      416   & NO  +             NO           & $\Longrightarrow$        & N$_2$  +         O$_2$     & 2.51e-11 & 0.00    & 30653.0  & UMIST     \\
      7601  & NH  +             O$_2$        & $\Longrightarrow$        & NO  +         OH           & 2.54e-14 & 1.18    & 312.0    & UMIST     \\
      \hline
      %       &                                & Radiative Dissociation   &                            &          &         &          &           \\
      % \hline
      % 3774  & NH                             & $\Longrightarrow$        & H   +         N            & 5.00e-10 & 0.00    & 2.3      & UMIST     \\
      % 3796  & C$_2$                          & $\Longrightarrow$        & C   +         C            & 2.40e-10 & 0.00    & 2.6      & UMIST     \\
      % 3803  & CN                             & $\Longrightarrow$        & C   +         N            & 2.90e-10 & 0.00    & 3.5      & UMIST     \\
      % 3811  & CO                             & $\Longrightarrow$        & C   +         O            & 2.00e-10 & 0.00    & 3.5      & UMIST     \\
      % 3812  & N$_2$                          & $\Longrightarrow$        & N   +         N            & 2.30e-10 & 0.00    & 3.9      & UMIST     \\
      % 3823  & NO                             & $\Longrightarrow$        & N   +         O            & 4.70e-10 & 0.00    & 2.1      & UMIST     \\
      % 3831  & O$_2$                          & $\Longrightarrow$        & O   +         O            & 7.90e-10 & 0.00    & 2.1      & UMIST     \\
      % \hline
            &                                & Collisional Dissociation &                            &          &         &          &           \\
      \hline
      194   & NH  +             NH           & $\Longrightarrow$        & H   +         H   +  N$_2$ & 1.16e-09 & 0.00    & 0.0      & UMIST     \\
      205   & NH  +             NO           & $\Longrightarrow$        & H   +         N$_2$  +  O  & 7.40e-10 & 0.00    & 10540.0  & UMIST     \\
      4060  & H   +             H$_2$        & $\Longrightarrow$        & H   +         H   +  H     & 4.67e-07 & -1.00   & 55000.0  & UMIST     \\
      4061  & CH  +             H            & $\Longrightarrow$        & C   +         H   +  H     & 6.00e-09 & 0.00    & 40200.0  & UMIST     \\
      4062  & H   +             OH           & $\Longrightarrow$        & H   +         H   +  O     & 6.00e-09 & 0.00    & 50900.0  & UMIST     \\
      4067  & H   +             O$_2$        & $\Longrightarrow$        & H   +         O   +  O     & 6.00e-09 & 0.00    & 52300.0  & UMIST     \\
      4069  & H$_2$  +             H$_2$     & $\Longrightarrow$        & H   +         H   +  H$_2$ & 1.00e-08 & 0.00    & 84100.0  & UMIST     \\
      4070  & CH  +             H$_2$        & $\Longrightarrow$        & C   +         H   +  H$_2$ & 6.00e-09 & 0.00    & 40200.0  & UMIST     \\
      4071  & H$_2$  +             OH        & $\Longrightarrow$        & H   +         H$_2$  +  O  & 6.00e-09 & 0.00    & 50900.0  & UMIST     \\
      4074  & H$_2$  +             O$_2$     & $\Longrightarrow$        & H$_2$  +         O   +  O  & 6.00e-09 & 0.00    & 52300.0  & UMIST     \\
      4076  & CO  +             M            & $\Longrightarrow$        & C   +         M   +  O     & 2.79e-03 & -3.52   & 128700.0 & BDDG76    \\
      7002  & CO  +             H            & $\Longrightarrow$        & C   +         H   +  O     & 2.79e-03 & -3.52   & 128700.0 & BDDG76    \\
      7585  & CH  +             O$_2$        & $\Longrightarrow$        & CO  +         H   +  O     & 1.14e-11 & 0.00    & 0.0      & UMIST     \\
      \hline
      \label{table:cno_rn}
\end{longtable}
\twocolumn

==> tables/metallicity_cemp_timescales.tex <==
% Table describing the cases and pathway timescales
\begin{table}[h!]
  \caption{Time-to-equilibrium for all models and key molecular species at a
    temperature of $3500$~K and a gas density of $10^{-9}$~g~cm$^{-3}$,
    corresponding to the upper photospheric convection cells. Due to
    the time-stepping of the solver, these times are not exact, but they provide
    a useful picture of how quickly various species set into equilibrium at
    varying chemical compositions.}
  \begin{center}
    \scalebox{0.85}{
      \begin{tabular}{ l r r r r r}
        \toprule
        Model & $t_\mathrm{eqm}$(C$_2$) & $t_\mathrm{eqm}$(CH) & $t_\mathrm{eqm}$(CN) & $t_\mathrm{eqm}$(CO) & $t_\mathrm{eqm}$(OH) \\
              & [s]                     & [s]                  & [s]                  & [s]                  & [s]                  \\
        \midrule
        AM1   & $4.5 \times 10^2$       & $1.0 \times 10^3$    & $2.4 \times 10^3$    & $1.7 \times 10^2$    & $1.7 \times 10^2$    \\
        AM2   & $5.7 \times 10^3$       & $5.1 \times 10^3$    & $6.3 \times 10^4$    & $3.9 \times 10^3$    & $3.2 \times 10^3$    \\
        AM3   & $4.9 \times 10^4$       & $2.4 \times 10^4$    & $2.4 \times 10^5$    & $4.0 \times 10^4$    & $1.3 \times 10^4$    \\
        \midrule
        AC1   & $9.0 \times 10^3$       & $7.7 \times 10^3$    & $1.6 \times 10^4$    & $1.6 \times 10^3$    & $1.6 \times 10^3$    \\
        AC2   & $2.2 \times 10^3$       & $1.2 \times 10^3$    & $2.4 \times 10^3$    & $1.8 \times 10^3$    & $2.4 \times 10^3$    \\
        \bottomrule
      \end{tabular}
    }
  \end{center}
  \label{table:metallicity_cemp_times}
\end{table}

==> tables/pathfinding_experiment.tex <==
% Table describing the cases and pathway timescales
\begin{table}[h!]
  \caption{Total timescales for the C-CH-CO pathway $P\subrm{1}$ and the
    O-OH-CO pathway $P\subrm{2}$ (towards formation of CO) for three different
    $\log$ C/O ratios.}
  \begin{center}
    \begin{tabular}{l c c r r r }
      \toprule
      Case & A(C)   & A(O)   & $\log$ C/O & $P\subrm{1}$   & $P\subrm{2}$   \\
           &        &        &            & [s]            & [s]            \\
      \midrule
      1    & $6.41$ & $7.06$ & $-0.65$    & $36.8$         & $\mathbf{1.6}$ \\
      2    & $7.06$ & $7.06$ & $0.00$     & $3.6 $         & $3.6$          \\
      3    & $7.06$ & $6.41$ & $+0.65$    & $\mathbf{1.6}$ & $36.8$         \\
      \bottomrule
    \end{tabular}
  \end{center}
  \label{table:pathfinding_timescales}
\end{table}

==> tables/rate_limiting_timescales.tex <==
% Table describing the cases and pathway timescales
\begin{table}[h!]
  \caption{Step-by-step reactions and rate-limiting steps for the AM3 model
    atmosphere at a temperature of $3500$ [K] and a gas density of $10^{-9}$
    [g cm$^{-3}$]. The rate-limiting step (longest step in a pathway), is
    highlighted in bold.}
  \begin{center}
    \scalebox{0.90}{
      \begin{tabular}{l r l c r l }
        \toprule
        Pathway            & Step & Reactants &               & Products  & Timescale [s]                  \\
        \midrule
        C $\rightarrow$ CO &      &           &               &           &                                \\
        \midrule
        \textbf{Pathway 1} & 1.   & C + OH    & $\rightarrow$ & CO + H    & $\mathbf{7.43 \times 10^{-5}}$ \\
                           &      &           &               & Total:    & $7.43 \times 10^{-5}$          \\
                           &      &           &               &           & ---------------                \\
        \textbf{Pathway 2} & 1.   & C + OH    & $\rightarrow$ & CH + O    & $\mathbf{4.10 \times 10^{-3}}$ \\
                           & 2.   & CH + O    & $\rightarrow$ & CO + H    & $4.27 \times 10^{-4}$          \\
                           &      &           &               & Total:    & $4.53 \times 10^{-3}$          \\
                           &      &           &               &           & ---------------                \\
        \textbf{Pathway 3} & 1.   & C + NO    & $\rightarrow$ & CN + O    & $\mathbf{1.44 \times 10^{1}}$  \\
                           & 2.   & CN + O    & $\rightarrow$ & CO + N    & $6.46 \times 10^{-3}$          \\
                           &      &           &               & Total:    & $1.44 \times 10^{1}$           \\
        \midrule
        O $\rightarrow$ CO &      &           &               &           &                                \\
        \midrule
        \textbf{Pathway 1} & 1.   & CH + O    & $\rightarrow$ & CO + H    & $\mathbf{4.27 \times 10^{-4}}$ \\
                           &      &           &               & Total:    & $4.27 \times 10^{-4}$          \\
                           &      &           &               &           & ---------------                \\
        \textbf{Pathway 2} & 1.   & CH + O    & $\rightarrow$ & C + OH    & $\mathbf{2.63 \times 10^{-3}}$ \\
                           & 2.   & C + OH    & $\rightarrow$ & CO + H    & $7.43 \times 10^{-5}$          \\
                           &      &           &               & Total:    & $2.70 \times 10^{-3}$          \\
                           &      &           &               &           & ---------------                \\
        \textbf{Pathway 3} & 1.   & O + C2    & $\rightarrow$ & C + CO    & $\mathbf{6.72 \times 10^{0}}$  \\
                           &      &           &               & Total:    & $6.72 \times 10^{0}$           \\
        \midrule
        CO $\rightarrow$ C &      &           &               &           &                                \\
        \midrule
        \textbf{Pathway 1} & 1.   & CO + H    & $\rightarrow$ & C + OH    & $\mathbf{6.26 \times 10^{-5}}$ \\
                           &      &           &               & Total:    & $6.26 \times 10^{-5}$          \\
                           &      &           &               &           & ---------------                \\
        \textbf{Pathway 2} & 1.   & CO + H    & $\rightarrow$ & C + O + H & $\mathbf{5.27 \times 10^{-1}}$ \\
                           &      &           &               & Total:    & $5.27 \times 10^{-1}$          \\
                           &      &           &               &           & ---------------                \\
        \textbf{Pathway 3} & 1.   & CO + M    & $\rightarrow$ & C + O + M & $\mathbf{5.24 \times 10^{0}}$  \\
                           &      &           &               & Total:    & $5.24 \times 10^{0}$           \\
        \midrule
        CO $\rightarrow$ O &      &           &               &           &                                \\
        \midrule
        \textbf{Pathway 1} & 1.   & CO + H    & $\rightarrow$ & C + OH    & $6.26 \times 10^{-5}$          \\
                           & 2.   & C + OH    & $\rightarrow$ & CH + H    & $\mathbf{4.10 \times 10^{-3}}$ \\
                           &      &           &               & Total:    & $4.16 \times 10^{-3}$          \\
                           &      &           &               &           & ---------------                \\
        \textbf{Pathway 2} & 1.   & CO + H    & $\rightarrow$ & C + O + H & $\mathbf{5.27 \times 10^{-1}}$ \\
                           &      &           &               & Total:    & $5.27 \times 10^{-1}$          \\
                           &      &           &               &           & ---------------                \\
        \textbf{Pathway 3} &      &           &               &           &                                \\
                           & 1.   & CO + C    & $\rightarrow$ & C2 + O    & $\mathbf{3.24 \times 10^{1}}$  \\
                           &      &           &               & Total:    & $3.24 \times 10^{1}$           \\
        \bottomrule
      \end{tabular}
    }
  \end{center}
  \label{table:rate_limiting}
\end{table}
